Mathematical and Statistical Opportunities in Cyber Security

The role of mathematics in a complex system such as the Internet has yet to be deeply explored. In this paper, we summarize some of the important and pressing problems in cyber security from the viewpoint of open science environments. We start by posing the question "What fundamental problems exist within cyber security research that can be helped by advanced mathematics and statistics?" Our first and most important assumption is that access to real-world data is necessary to understand large and complex systems like the Internet. Our second assumption is that many proposed cyber security solutions could critically damage both the openness and the productivity of scientific research. After examining a range of cyber security problems, we come to the conclusion that the field of cyber security poses a rich set of new and exciting research opportunities for the mathematical and statistical sciences.

==> Notes.tex <==
Network traffic is often modeled as a Poisson process because they have good theoretical properties.  Studies have shown however that the Poisson model does not hold for real network traffic including both local area and wide area network traffic.  One study~\cite{LTWW94}  makes a case that local area network can be modeled much better as a self-similar process.  For an excellent survey on self-similar traffic modeling and analysis see~\cite{WiTaEr96}. In~cite{Paxson1995} suggest that the Poisson-based models should also be abandoned for wide-area traffic.   As a result, Willinger and Paxson~\cite{?} point out that there is a need for the development of statistical techniques and methods for  effectively  handling phenomena such as heavy tails and long-range dependence that have been empirically observed in network traffic data.
 
One of the main goals in intrusion and anomaly detection is ...
Several approaches have been proposed including,  support vector regresssion~\cite{Mirza07},k-means~\cite{Lakhina2005}, multivariate adaptive regression splines~\cite{Mukkamala}, and sequential hypothesis testing~\cite{Jung}.  As the data set sizes increase and the need to more quickly detect intrusions, more robust, accurate, and efficient algorithms will be required.

